FashionNTM: Multi-turn Fashion Image Retrieval via Cascaded Memory

Multi-turn textual feedback-based fashion image retrieval focuses on a real-world setting, where users can iteratively provide information to refine retrieval results until they find an item that fits all their requirements. In this work, we present a novel memory-based method, called FashionNTM, for such a multi-turn system. Our framework incorporates a new Cascaded Memory Neural Turing Machine (CM-NTM) approach for implicit state management, thereby learning to integrate information across all past turns to retrieve new images, for a given turn. Unlike vanilla Neural Turing Machine (NTM), our CM-NTM operates on multiple inputs, which interact with their respective memories via individual read and write heads, to learn complex relationships. Extensive evaluation results show that our proposed method outperforms the previous state-of-the-art algorithm by 50.5%, on Multi-turn FashionIQ -- the only existing multi-turn fashion dataset currently, in addition to having a relative improvement of 12.6% on Multi-turn Shoes -- an extension of the single-turn Shoes dataset that we created in this work. Further analysis of the model in a real-world interactive setting demonstrates two important capabilities of our model -- memory retention across turns, and agnosticity to turn order for non-contradictory feedback. Finally, user study results show that images retrieved by FashionNTM were favored by 83.1% over other multi-turn models. Project page: https://sites.google.com/eng.ucsd.edu/fashionntm

==> tables/ablation_memory_size.tex <==
\begin{table}[t]
\scriptsize
\centering
\caption{Ablation study 1: Different memory size configurations for the proposed memory network approach by fixing the number of cascaded memories to $2$. We pick the best setting of memory size from this table and use it for other ablation studies.}
\label{tab:mem_size_ablation}
\begin{tabular}{c|cccccc}\toprule
Memory size && R@$5$ & R@$8$ & Mean\\
\hline
% $1 \times 768$ && $25.47$ & $33.33$ & $29.38$\\
$2 \times 768$ && $24.52$ & $31.42$ & $27.97$\\
$4 \times 768$ && $24.52$ & $30.47$ & $27.49$\\
$8 \times 768$ && $\mathbf{25.71}$ & $\mathbf{33.33}$ & $\mathbf{29.5}$\\
$16 \times 768$ && $25.23$ & $32.14$ & $28.68$\\
% $32 \times 768$ && \textbf{$9.5$} & $26.9$ & \textbf{$34.8$} & \textbf{$23.8$}\\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}

==> tables/ablation_study.tex <==
\begin{table*}[t]
\scriptsize
\centering
\caption{Ablation study}
\label{tab:ablation}
\begin{tabular}{cccccccccccccccccccc}\toprule
\multirow{3}{*}{\parbox{1cm}{Memory size}} & \multicolumn{19}{c}{Number of memories}\\
\cline{2-20}
& \multicolumn{3}{c}{$1$} && \multicolumn{3}{c}{$2$} && \multicolumn{3}{c}{$4$} && \multicolumn{3}{c}{$8$} && \multicolumn{3}{c}{$16$} \\
\cline{2-4} \cline{6-8} \cline{10-12} \cline{14-16} \cline{18-20}
& R@$1$ & R@$5$ & R@$8$ && R@$1$ & R@$5$ & R@$8$ && R@$1$ & R@$5$ & R@$8$ && R@$1$ & R@$5$ & R@$8$ && R@$1$ & R@$5$ & R@$8$ \\
\hline
$1 \times 768$ & $10.2$ & $25.0$ & $34.5$ && $8.1$ & $26.2$ & $33.6$ && $9.5$ & $27.4$ & $33.1$ && $8.6$ & $29.3$ & $34.3$ && $8.6$ & $26.2$ & $33.3$ \\ 
$2 \times 768$ & $10.5$ & $26.4$ & $32.4$ && $8.3$ & $26.9$ & $33.8$ && $8.8$ & $27.4$ & $32.1$ && $8.3$ & $26.2$ & $33.3$ && $8.8$ & $26.2$ & $34.3$ \\ 
$4 \times 768$ & $8.6$ & $27.1$ & $34.3$ && $9.3$ & $26.4$ & $33.8$ && $8.6$ & $27.6$ & $35.5$ && $8.3$ & $26.9$ & $35.2$ && $11.0$ & $26.4$ & $33.8$ \\ 
$8 \times 768$ & $10.7$ & $27.1$ & $33.6$ && $8.8$ & $26.2$ & $33.3$ && $7.6$ & $26.7$ & $35.7$ && $9.8$ & $28.3$ & $34.0$ && $10.2$ & $27.1$ & $33.8$ \\ 
$16 \times 768$ & $10.5$ & $27.6$ & $33.8$ && $8.8$ & $27.3$ & $33.6$ && $7.6$ & $26.9$ & $35.5$ && $10.2$ & $28.8$ & $33.3$ && $9.8$ & $27.9$ & $33.8$ \\ 
$32 \times 768$ & $8.8$ & $26.0$ & $35.7$ && $9.5$ & $26.9$ & $34.8$ && $7.8$ & $26.4$ & $34.5$ && $8.8$ & $26.4$ & $34.6$ && $10.5$ & $26.7$ & $34.0$ \\ 
$64 \times 768$ & $11.4$ & $27.4$ & $35.2$ && $9.5$ & $26.9$ & $32.6$ && $10.2$ & $28.1$ & $32.9$ && $11.4$ & $25.7$ & $34.0$ && $9.8$ & $27.6$ & $34.5$ \\ 
\cline{2-4} \cline{6-8} \cline{10-12} \cline{14-16} \cline{18-20}
Mean & \multicolumn{3}{c}{$30.4$} && \multicolumn{3}{c}{$30.2$} && \multicolumn{3}{c}{$\mathbf{30.7}$} && \multicolumn{3}{c}{$\mathbf{30.7}$} && \multicolumn{3}{c}{$30.4$} \\ 
\bottomrule
\end{tabular}
\end{table*}

==> tables/shoes_dataset_stat.tex <==
\begin{table}[t]
\scriptsize
\centering
\caption{Reduction in dataset size with increasing turn length.}
\vspace{-10pt}
\label{tab:shoes_dataset_stat}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l|rrrrrr}\toprule
 &  & \multicolumn{4}{c}{\textbf{Number of transactions with}}\\
 \cline{3-6}
\textbf{Dataset} & \textbf{Split} & \textbf{$2$-turns} & \textbf{$3$-turns} & \textbf{$4$-turns} & \textbf{\textcolor{red}{$5$-turns}}\\
\hline
Multi-turn & Train & $1,659$ & $1,036$ & $982$ & $\textcolor{red}{358}$ \\
Shoes (ours) & Test & $296$ & $96$ & $28$ & $\textcolor{red}{3}$ \\
\bottomrule
\end{tabular}
\vspace{-15pt}
\end{table}
